BCFW recursion for off-shell gluons

It is shown how tree-level multi-gluon helicity amplitudes with an arbitrary number of off-shell external gluons can be calculated via BCFW recursion. Compact expressions for helicity amplitudes for scattering processes of three and four gluons, with up to three of them off-shell, are presented. Also, maximum-helicity-violating configurations are identified for up to two off-shell gluons, and the expressions for their helicity amplitudes for an arbitrary number of on-shell gluons are derived.

==> 5_examples_4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{$\emptyset\to g^*g^*g^*g$}
There are four non-vanishing contributions to $\Amp(1^*,2^*,3^+,4^*)$.
%
The first is
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\graph{graph43}{10}{3.8}\!\!\frac{1}{K_{3,4}^2}\!\graph{graph44}{10}{3.8}
=
\frac{1}{\kstr_1\kstr_2}\,\frac{\AA{12}^3}{\AA{2\hat{K}}\AA{\hat{K}3}}
\,\frac{1}{(p_3+k_4)^2}\,\frac{1}{\kapp_4}\,\frac{\SSS{43}^3}{\SSS{3\hat{K}}\SSS{\hat{K}4}}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


